Local Coarsening Algorithms on Adaptively Refined Meshes in 2D and Their Efficient Implementation in MATLAB

Adaptive meshing includes local refinement as well as coarsening of meshes. Typically, coarsening algorithms are based on an explicit refinement history. In this work, we deal with local coarsening algorithms that build on the refinement strategies for triangular and quadrilateral meshes implemented in the ameshref package (Funken and Schmidt 2018, 2019). The ameshref package is a MATLAB-toolbox for research and teaching purposes which offers the user a certain flexibility in the REFINE step of an adaptive finite element method but can also be used in other contexts like computer graphics. This toolbox is now be extended by the coarsening option. In ameshref, no explicit information about the refinement process is stored, but is instead implicit in the data structure. In this work, we present coarsening algorithms that use easy-to-verify criteria to coarsen adaptively generated meshes by exploiting the data structure. Thereby, the desired properties are guaranteed and computational efficiency is maintained. A MATLAB implementation and some numerical examples are discussed in this work and are included in full in the toolbox ameshcoars (Funken and Schmidt 2020).

==> figures/TrefineRGBpattern.tex <==

\begin{figure}
\begin{minipage}[t]{0.19\linewidth}
\hspace*{6mm}\begin{tikzpicture}
[ interface/.style={
        % The border decoration is a path replacing decorator. 
        % For the interface style we want to draw the original path.
        % The postaction option is therefore used to ensure that the
        % border decoration is drawn *after* the original path.
        postaction={draw,decorate,decoration={border,angle=45,
                    amplitude=0.13cm,segment length=1mm}}},
    ]
\coordinate (1) at (-1.2,0);
\coordinate (2) at (1.2,0);
\coordinate (3) at (0,1.5);
\draw(1)--(2) -- (3)--(1);
\draw [interface, thick](1) --(2);
\fill (1) circle (2pt); 
\fill (2) circle (2pt); 
\fill (3) circle (2pt); 
\node at (0,-0.5) {none};
\end{tikzpicture}
\end{minipage}
\begin{minipage}[t]{0.19\linewidth}
\hspace*{6mm}\begin{tikzpicture}[ interface/.style={
        % The border decoration is a path replacing decorator. 
        % For the interface style we want to draw the original path.
        % The postaction option is therefore used to ensure that the
        % border decoration is drawn *after* the original path.
        postaction={draw,decorate,decoration={border,angle=45,
                    amplitude=0.13cm,segment length=1mm}}},
    ]
\coordinate (1) at (-1.2,0);
\coordinate (2) at (1.2,0);
\coordinate (3) at (0,1.5);
\draw[fill=lightgreen] (1) --(2)--(3)--(1);
\draw[interface,thick] (2) -- (3);
\draw[interface,thick] (3) -- (1);
\fill (1) circle (2pt); 
\fill (2) circle (2pt); 
\fill (3) circle (2pt); 
\fill ($(1)!0.5!(2)$) circle (2pt);
\draw ($(1)!0.5!(2)$) --(3);
%\node at (-0.4,0.35) {1};
%\node at (0.4,0.35) {2};
\node at (0,-0.5) {green};
\end{tikzpicture}
\end{minipage}
\begin{minipage}[t]{0.19\linewidth}
\hspace*{6mm}\begin{tikzpicture}[ interface/.style={
        % The border decoration is a path replacing decorator. 
        % For the interface style we want to draw the original path.
        % The postaction option is therefore used to ensure that the
        % border decoration is drawn *after* the original path.
        postaction={draw,decorate,decoration={border,angle=45,
                    amplitude=0.13cm,segment length=1mm}}},
    ]
\coordinate (1) at (-1.2,0);
\coordinate (2) at (1.2,0);
\coordinate (3) at (0,1.5);
\draw[fill=lightblue] (1)--(2) -- (3)--(1);
\draw[interface,thick] (3) -- (1);
\fill (1) circle (2pt); 
\fill (2) circle (2pt); 
\fill (3) circle (2pt); 
\fill ($(1)!0.5!(2)$) circle (2pt);
\fill ($(2)!0.5!(3)$) circle (2pt);
\draw ($(2)!0.5!(3)$) -- ($(1)!0.5!(2)$);
\draw[interface,thick] (3)--($(1)!0.5!(2)$);
\draw[interface,thick] ($(1)!0.5!(2)$) --(2);
\node at (0,-0.5) {blue$_r$};
%\node at (-0.4,0.35) {1};
%\node at (0.6,0.35) {2};
%\node at (0.3,0.75) {3};
\end{tikzpicture}
\end{minipage}
\begin{minipage}[t]{0.19\linewidth}
\hspace*{6mm}\begin{tikzpicture}[ interface/.style={
        % The border decoration is a path replacing decorator. 
        % For the interface style we want to draw the original path.
        % The postaction option is therefore used to ensure that the
        % border decoration is drawn *after* the original path.
        postaction={draw,decorate,decoration={border,angle=45,
                    amplitude=0.13cm,segment length=1mm}}},
    ]
\coordinate (1) at (-1.2,0);
\coordinate (2) at (1.2,0);
\coordinate (3) at (0,1.5);
\draw[fill=lightblue] (1)--(2) -- (3)--(1);
\draw[interface,thick] (2) -- (3);
\fill (1) circle (2pt); 
\fill (2) circle (2pt); 
\fill (3) circle (2pt); 
\fill ($(1)!0.5!(2)$) circle (2pt);
\fill ($(1)!0.5!(3)$) circle (2pt);
\draw ($(1)!0.5!(3)$) -- ($(1)!0.5!(2)$);
\draw[interface,thick] ($(1)!0.5!(2)$)--(3);
\draw[interface,thick] (1)-- ($(1)!0.5!(2)$);
\node at (0,-0.5) {blue$_\ell$};
%\node at (0.4,0.35) {3};
%\node at (-0.6,0.35) {2};
%\node at (-0.3,0.75) {1};
\end{tikzpicture}
\end{minipage}
\begin{minipage}[t]{0.19\linewidth}
\hspace*{6mm}\begin{tikzpicture}[ interface/.style={
        % The border decoration is a path replacing decorator. 
        % For the interface style we want to draw the original path.
        % The postaction option is therefore used to ensure that the
        % border decoration is drawn *after* the original path.
        postaction={draw,decorate,decoration={border,angle=45,
                    amplitude=0.13cm,segment length=1mm}}},
    ]
\coordinate (1) at (-1.2,0);
\coordinate (2) at (1.2,0);
\coordinate (3) at (0,1.5);
\draw[fill=pastelred] (1)--(2) -- (3)--(1);
\draw[interface,thick] (1) --(2);
\fill (1) circle (2pt); 
\fill (2) circle (2pt); 
\fill (3) circle (2pt); 
\fill ($(1)!0.5!(2)$) circle (2pt);
\fill ($(2)!0.5!(3)$) circle (2pt);
\fill ($(1)!0.5!(3)$) circle (2pt);
\draw ($(1)!0.5!(2)$) -- ($(2)!0.5!(3)$)--($(1)!0.5!(3)$)--($(1)!0.5!(2)$);
\draw[interface,thick] ($(2)!0.5!(3)$)--($(1)!0.5!(3)$);
\draw[interface,thick] ($(1)!0.5!(3)$)--($(2)!0.5!(3)$);
%\node at (-0.6,0.35) {1};
%\node at (0.6,0.35) {2};
%\node at (0,1.15) {3};
%\node at (0,0.35) {4};
\node at (0,-0.5) {red};
\end{tikzpicture}
\end{minipage}
\caption{Refinements red, green, blue$_r$, and blue$_\ell$. Reference edges are highlighted by hatched lines.}
\label{fig:RGB}
\end{figure}

==> figures/qrefinergquad1.tex <==

%\centering
\hspace*{2.3cm}
\begin{minipage}[t]{0.2\textwidth}
\begin{tikzpicture}
\coordinate (1) at (-0.5,-0.5);
\coordinate (2) at (1,-0.5);
\coordinate (3) at (1,1);
\coordinate (4) at (-0.5,1);
\coordinate(9) at (0.25,0.25);
\draw[fill=pastelred] (1) --(2)--(3)--(4)--(1);
\node[circle,draw=black, fill=white, inner sep=0pt,minimum size=4pt] at (1) {};
\node[circle,draw=black, fill=white, inner sep=0pt,minimum size=4pt] at (2) {};
\node[circle,draw=black, fill=white, inner sep=0pt,minimum size=4pt] at (3) {};
\node[circle,draw=black, fill=white, inner sep=0pt,minimum size=4pt] at (4) {};
\fill ($(4)!0.5!(1)$)  circle (2pt); 
\fill ($(2)!0.5!(1)$)  circle (2pt); 
\fill ($(3)!0.5!(2)$)  circle (2pt); 
\fill ($(4)!0.5!(3)$)  circle (2pt); 
\fill (9)  circle (2pt); 
\draw ($(4)!0.5!(1)$)--($(3)!0.5!(2)$);
\draw ($(2)!0.5!(1)$)--($(4)!0.5!(3)$);

\node at (0.25,-1) {red};
\end{tikzpicture}
\end{minipage}
\hspace*{-5mm}
\begin{minipage}[t]{0.2\textwidth}
\begin{tikzpicture}
\coordinate (1) at (-0.5,-0.5);
\coordinate (2) at (1,-0.5);
\coordinate (3) at (1,1);
\coordinate (4) at (-0.5,1);
\coordinate (5) at (0.25,0.25);
\draw[fill=lightblue] (1)--(2)--(3)--(4)--(1);
\draw ($(1)!0.5!(2)$)--(5)--($(2)!0.5!(3)$);
\draw (5)--(4);
\node[circle,draw=black, fill=white, inner sep=0pt,minimum size=4pt] at (1) {};
\fill (2) circle (2pt);
\fill (3) circle (2pt);
\fill (4) circle (2pt);
\fill (5) circle (2pt);
\fill ($(1)!0.5!(2)$) circle (2pt);
\fill ($(2)!0.5!(3)$) circle (2pt);
\node at (0.25,-1) {blue$_{r}$};
\end{tikzpicture}
\end{minipage}
\begin{minipage}[t]{0.2\textwidth}
\begin{tikzpicture}
\coordinate (1) at (-0.5,-0.5);
\coordinate (2) at (1,-0.5);
\coordinate (3) at (1,1);
\coordinate (4) at (-0.5,1);
\coordinate (5) at (0.25,0.25);
\draw[fill=lightblue] (1)--(2)--(3)--(4)--(1);
\draw ($(4)!0.5!(1)$)--(5)--($(4)!0.5!(3)$);
\draw (5)--(2);
\node[circle,draw=black, fill=white, inner sep=0pt,minimum size=4pt] at (1) {};
\fill (4) circle (2pt);
\fill (2) circle (2pt);
\fill (3) circle (2pt);
\fill (5) circle (2pt);
\fill ($(4)!0.5!(1)$) circle (2pt);
\fill ($(4)!0.5!(3)$) circle (2pt);
\node at (0.25,-1) {blue$_{\ell}$};
\end{tikzpicture}
\end{minipage}
\captionof{figure}{Red-blue refinement patterns.}
\label{fig:QRB}

